Large Language Models are Zero-Shot Reasoners

Pretrained large language models (LLMs) are widely used in many sub-fields of natural language processing (NLP) and generally known as excellent few-shot learners with task-specific exemplars. Notably, chain of thought (CoT) prompting, a recent technique for eliciting complex multi-step reasoning through step-by-step answer examples, achieved the state-of-the-art performances in arithmetics and symbolic reasoning, difficult system-2 tasks that do not follow the standard scaling laws for LLMs. While these successes are often attributed to LLMs' ability for few-shot learning, we show that LLMs are decent zero-shot reasoners by simply adding "Let's think step by step" before each answer. Experimental results demonstrate that our Zero-shot-CoT, using the same single prompt template, significantly outperforms zero-shot LLM performances on diverse benchmark reasoning tasks including arithmetics (MultiArith, GSM8K, AQUA-RAT, SVAMP), symbolic reasoning (Last Letter, Coin Flip), and other logical reasoning tasks (Date Understanding, Tracking Shuffled Objects), without any hand-crafted few-shot examples, e.g. increasing the accuracy on MultiArith from 17.7% to 78.7% and GSM8K from 10.4% to 40.7% with large InstructGPT model (text-davinci-002), as well as similar magnitudes of improvements with another off-the-shelf large model, 540B parameter PaLM. The versatility of this single prompt across very diverse reasoning tasks hints at untapped and understudied fundamental zero-shot capabilities of LLMs, suggesting high-level, multi-task broad cognitive capabilities may be extracted by simple prompting. We hope our work not only serves as the minimal strongest zero-shot baseline for the challenging reasoning benchmarks, but also highlights the importance of carefully exploring and analyzing the enormous zero-shot knowledge hidden inside LLMs before crafting finetuning datasets or few-shot exemplars.

==> OLD2_table_related_work.tex <==
\begin{table}[t]\centering
\scriptsize
%\footnotesize
%\fontsize{9pt}{0.1cm}\selectfont
%\begin{tabular}{lllllll}
\begin{tabular}{|p{0.23\textwidth}|p{0.09\textwidth}|p{0.11\textwidth}|p{0.06\textwidth}|p{0.16\textwidth}|p{0.06\textwidth}|}
%\begin{tabular}{lrrrrr}\toprule
\toprule

Method &Category &Task Family&Versatile Prompt? &Model &Output CoT?  \\\midrule
\cite{yourself} &Fine-Tuning &Reasoning & &GPT &$\checkmark$ \\
\cite{gsm8k} &Fine-Tuning &Reasoning & &GPT-3 &$\checkmark$ \\
\cite{star} &Fine-Tuning &Reasoning & &GPT-3, etc &$\checkmark$ \\
\cite{scratchpad} &Fine-Tuning &Reasoning & &Transformer(Decoder) &$\checkmark$ \\

\midrule

\cite{brown2020language} &Few-Shot &Reasoning & &GPT-3 & \\
\cite{megatron} &Few-Shot &Reasoning & &MT-NLG & \\
\cite{gopher} &Few-Shot &Reasoning  & &Gopher & \\
\cite{cot_wei} &Few-Shot &Reasoning& &PaLM, etc  &$\checkmark$ \\
\cite{cot_wei_sc} &Few-Shot &Reasoning & &PaLM, etc  &$\checkmark$\\
\cite{palm} &Few-Shot &Reasoning& &PaLM  &$\checkmark$ \\

\midrule

\cite{selftalk} &Zero-Shot &Reasoning& &GPT-2, etc  &$\checkmark$ \\
\cite{prompt1} &Zero-Shot &Reasoning& &GPT-3  &$\checkmark$ \\
\ours (Ours) &Zero-Shot &Reasoning&$\checkmark$ &GPT-3  &$\checkmark$ \\
\bottomrule
\end{tabular}

%\begin{tabular}{|p{0.23\textwidth}|p{0.09\textwidth}|p{0.11\textwidth}|p{0.06\textwidth}|p{0.25\textwidth}|}
%\toprule
%%\begin{tabular}{lrrrr}\toprule
%Method &Category &Task Family & Versatile Prompt? &Prompt example \\\midrule
%\cite{Radford2019LanguageMA} &Zero-Shot &Summarization &$\checkmark$  &TL;DR \\
%\cite{cando} &Zero-Shot &Robotics &$\checkmark$  &First, \\
%\cite{prompt1} &Zero-Shot &Reasoning &  &Let's solve this problem by splitting it into steps. \\
%\cite{prompt1} &Zero-Shot &Translation &  &The masterful French translator flawlessly translates the phrase into English: \\
%&Zero-Shot &Text-to-Image &$\checkmark$  &unreal engine \\
%% \cite{selfdiagnosis} &Zero-Shot &Toxic &$\checkmark$  &Two guys in a bar start a \\
%% \cite{realtoxicityprompts} &Zero-Shot &Toxic &$\checkmark$  &I'm 99 \% sure it was someone being an \\
%% \cite{generating} &Zero-Shot &Similarity &$\checkmark$  &Write two sentences that \\
%\bottomrule
%\end{tabular}

\captionsetup{skip=5pt}
\caption{Related work focusing on arithmetic or commonsense reasoning tasks. \ours is the only method that proposes and validates the versatility of single prompt for solving a wide variety of reasoning tasks with \CoT reasoning. 
% Bottom) Related work that proposed zero-shot versatile prompts from other task families besides reasoning. Like \ours, these prompts are universally useful and do not need to be engineered differently per task in the task family. Critically, only the non-trivial prefix prompts are listed in this bottom table, and all these prior works do not systematically evaluate the extensiveness of these generic prompts as thoroughly done as in our work.

%\sg{note1: if Notes have sparse entries, remove that from the table, and just add footnotes.} 
%\sg{note2: i actually want a complete survey on all representative prompting works beyond those in arithmetic or commonsense reasoning; add "Tasks" column. besides ours, are there any prompts that work on multiple tasks? if not, we can make very strong statements.} \mr{it might make more sense to have one row for each combination instead of having each work on it's own row?} \sg{to mr: i like that}
}
\label{tab:related_work}
\end{table}


\begin{table}[t]
\centering
\caption{Test Table}\label{tab: }
%\footnotesize
\scriptsize
\begin{tabular}
%{llllll}
{|p{0.12\textwidth}|p{0.12\textwidth}|p{0.12\textwidth}|p{0.15\textwidth}|p{0.30\textwidth}|}
\toprule
Category &Prompt Setting &Implicit / Explicit Reasoning &\# of Demonstrations &Method (Model) \\\midrule
Fine-Tuning &- &Implicit or \par Explicit &Large or Few \par (with CoT text) &\cite{yourself} (GPT) \par \cite{gsm8k} (GPT-3) \par \cite{star} (GPT-3, etc) \par \cite{scratchpad} (Transformer(Decoder)) \\

\midrule

\theirsf &Example-base &Implicit &Few &\cite{brown2020language} (GPT-3) \par \cite{megatron} (MT-NLG) \par \cite{gopher} (Gopher) \\

\midrule

\theirs &Example-base &Explicit &Few \par (with CoT text) &\cite{cot_wei} (PaLM, etc) \par \cite{cot_wei_sc} (PaLM, etc) \par \cite{palm} (PaLM) \\

\midrule

\theirsz &Template-base &Implicit &Zero &- \\

\midrule

\ours &Template-base &Explicit &Zero &\cite{selftalk}(GPT-2) \par \cite{prompt1}(GPT-3) \par \ours (Ours)(GPT-3) \\
\bottomrule
\end{tabular}
\end{table}




==> OLD_table_algorithm.tex <==
\begin{algorithm}[t]
\caption{\ours}
\label{alg:algorithm}
\textbf{Input}: 
Question x $\in$ X, pre-trained model M, First template $\tau_1$, Second template $\tau_2$ \\
\textbf{Output}:
\begin{algorithmic}[1]
\STATE {pred\_list=[]}
\FOR{each x in X}
\STATE x’ $\leftarrow$ $\tau_1$(x)
\STATE z $\leftarrow$ M(x’)
\STATE z’ $\leftarrow$ $\tau_2$(x', z)
\STATE y' $\leftarrow$ M(z’)
\STATE $\hat{y}$ $\leftarrow$ Answer Cleansing(y')
\STATE pred\_list.append($\hat{y}$)
\ENDFOR
\RETURN pred\_list
\end{algorithmic}
\end{algorithm}

==> OLD_table_related_work.tex <==
\begin{table}[t]\centering
\scriptsize
%\begin{tabular}{lllllll}
\begin{tabular}{|p{0.23\textwidth}|p{0.18\textwidth}|p{0.06\textwidth}|p{0.06\textwidth}|p{0.23\textwidth}|}
\toprule
Method &Category &Use CoT? & Versatile &Notes \\\hline \hline
\cite{gsm8k} &Fine-Tuning &$\checkmark$ & & \\\hline
\cite{yourself} &Fine-Tuning &$\checkmark$ & & \\\hline
\cite{star} &Fine-Tuning &$\checkmark$ & &This method auguments CoT samples by Few-shot approach \cite{cot_wei}. \\\hline
\cite{scratchpad} &Fine-Tuning &$\checkmark$ & & \\\hline
\hline
\cite{gpt3} &Few-Shot Prompt & & & \\\hline
\cite{megatron} &Few-Shot Prompt & & &\\\hline
\cite{gopher} &Few-Shot Prompt & & & \\\hline
\cite{palm} &Few-Shot Prompt &$\checkmark$ & & \\\hline
\cite{cot_wei} &Few-Shot Prompt &$\checkmark$ & & \\\hline
\cite{cot_wei_sc} &Few-Shot Prompt &$\checkmark$ & & \\\hline
\hline
\cite{selftalk} &Zero-Shot Prompt & & &Limited prompting approach \\\hline
\cite{prompt1} &Zero-Shot Prompt & & &Samples are illustrated but no quantitative experiments. \\\hline
Ours &Zero-Shot Prompt & $\checkmark$ &$\checkmark$ & \\
\hline
\end{tabular}
\captionsetup{skip=5pt}
\caption{Related work focusing on arithmetic or commonsense reasoning tasks. CoT : An approach utilizing \CoT reasoning, Non-CoT : An approach which does not utilize \CoT reasoning. \sg{note1: if Notes have sparse entries, remove that from the table, and just add footnotes.} \sg{note2: i actually want a complete survey on all representative prompting works beyond those in arithmetic or commonsense reasoning; add "Tasks" column. besides ours, are there any prompts that work on multiple tasks? if not, we can make very strong statements.} \mr{it might make more sense to have one row for each combination instead of having each work on it's own row?} \sg{to mr: i like that}}
\label{tab:related_work}
\end{table}


==> table_palm_algorithm.tex <==
\begin{algorithm}[h]
\caption{\oursvtwo + Self-Consistency}
\label{alg:algorithm_palm}
\textbf{Input}: 
Questions $X$ for test dataset; pretrained language model $M$; reasoning extraction template $\tau_{r}$ and answer extraction template $\tau_a$ for \ours; number of few-shot prompt templates $N_p$; number of exemplars per few-shot prompt template $N_e$; number of text output samples per few-shot prompt template $N_a$ using random sampling strategy K\\
\textbf{Output}: Answer predictions ${\hat{Y}}$ for test dataset
\begin{algorithmic}[1]
\STATE \textit{\textbf{\# Exemplar Creation}} \algcomment{$N_p*N_e$ questions are evaluated using \ours}
\STATE $P = \emptyset$ \algcomment{\# Initialize an empty set of few-shot prompt templates}
\FOR{each $i=1\rightarrow N_p$}
\STATE $P_i = $``'' \algcomment{\# Initialize an empty string for a few-shot template}
\FOR{each $j=1\rightarrow N_e$}
\STATE Randomly sample a question $x\sim X$
\STATE $x' \leftarrow \tau_r(x)$ \algcomment{ \# Create a prompt for reasoning extraction}
\STATE $z\leftarrow GreedyDecoding(x'; M)$ \algcomment{ \# Reasoning extraction}
\STATE $z'\leftarrow$ $\tau_a(x', z)$ \algcomment{\# Create a prompt for answer extraction}
\STATE $\hat{y} \leftarrow GreedyDecoding(z'; M)$ \algcomment{\# Answer extraction}
\STATE $P_i \leftarrow Concat(P_i, z', \hat{y})$ \algcomment{\# Concatenate question, reasoning, answer as an exemplar and append to the few-shot template}
\ENDFOR
\STATE $P \leftarrow P \cup P_i$ \algcomment{ \# Store the created few-shot template into list}
\ENDFOR
\STATE
\STATE \textit{\textbf{\# Self-Consistency}} \algcomment{$N_p*N_a$ samples are generated per question}
\STATE {$\hat{Y} = \emptyset$}
\FOR{each $x$ in $X$}
\STATE {$\Omega = \emptyset$}
\STATE \lighttext{\# Generate $N_p * N_a$ reasoning paths by random sampling}
\FOR{each $k = 1 \rightarrow N_p$}
\FOR{each $l = 1 \rightarrow N_a$}
\STATE $z \leftarrow RandomSampling(x, P_i; M, K)$ \algcomment{ \# Random sampling}
\STATE \lighttext{\# Answer extraction prompting is no more needed thanks to self-created exemplars}
\STATE $\hat{y} \leftarrow ParseAnswer(z)$
\STATE $\Omega \leftarrow \Omega \cup \hat{y}$
\ENDFOR
\ENDFOR
\STATE $\Tilde{y} \leftarrow Mode(\Omega)$ \algcomment{\# Majority Voting}
\STATE $\hat{Y} \leftarrow \hat{Y} \cup \Tilde{y}$
\ENDFOR
\end{algorithmic}
\end{algorithm}
